On an Improvement over R\'enyi's Equivocation Bound

We consider the problem of estimating the probability of error in multi-hypothesis testing when MAP criterion is used. This probability, which is also known as the Bayes risk is an important measure in many communication and information theory problems. In general, the exact Bayes risk can be difficult to obtain. Many upper and lower bounds are known in literature. One such upper bound is the equivocation bound due to R\'enyi which is of great philosophical interest because it connects the Bayes risk to conditional entropy. Here we give a simple derivation for an improved equivocation bound. We then give some typical examples of problems where these bounds can be of use. We first consider a binary hypothesis testing problem for which the exact Bayes risk is difficult to derive. In such problems bounds are of interest. Furthermore using the bounds on Bayes risk derived in the paper and a random coding argument, we prove a lower bound on equivocation valid for most random codes over memoryless channels.

==> Makefile <==
#################################################################################
#################################################################################
##
## Author: Nandakishore Santhi (nsanthi@ucsd.edu)
##
## This Makefile is meant for use with the following LaTeX(2e) systems:
## (1) Linux + GNU make + (pdf)LaTeX
## (2) Windows + GNU make + MiKTeX
## (3) Windows + cygwin + GNU make + (pdf)LaTeX
##
#################################################################################
#################################################################################
FILE=equivocation
#Use for Windows + MiKTeX
#TEXOPTIONS=-include-directory=. -include-directory=Styles -include-directory=Sections
#Use for Linux/Unix
TEXOPTIONS=
LATEX=TEXINPUTS=.//:./Styles//:./Sections//:./Support: latex ${TEXOPTIONS}
PDFLATEX=TEXINPUTS=.//:./Styles//:./Sections//:./Support: pdflatex ${TEXOPTIONS}
BIBTEX=bibtex
SOURCES=equivocation.tex \
		MyMacros.tex \
		MyBiblio.bib

all: ${SOURCES} Makefile
	@make -s pdf ps
	@echo "___________________________________________________________"
	@echo "Check for errors in out_bib.log out_ps.log and out_pdf.log!"
	@echo "___________________________________________________________"

dvi: ${FILE}.dvi
${FILE}.dvi: ${SOURCES}
	${LATEX} ${FILE}.tex
	${BIBTEX} ${FILE} > out_bib.log
	${LATEX} ${FILE}.tex
	${LATEX} ${FILE}.tex
	${LATEX} ${FILE}.tex > out_ps.log

pdf: ${FILE}.pdf
${FILE}.pdf: ${SOURCES}
	@echo "Patience Pays!"
	${PDFLATEX} ${FILE}.tex
	${BIBTEX} ${FILE} > out_bib.log
	${PDFLATEX} ${FILE}.tex
	${PDFLATEX} ${FILE}.tex
	${PDFLATEX} ${FILE}.tex > out_pdf.log
	@echo "___________________________________________________________"

ps: ${FILE}.ps
${FILE}.ps: ${SOURCES}
	@echo "Patience Pays Again!"
	@make dvi
	dvips -Z -V -t letter ${FILE}.dvi -o ${FILE}.ps
	#pdf2ps -dSubsetFonts=true -dPDFSETTINGS=/printer -dEmbedAllFonts=true -dOptimize=true -dEmbedAll=true ${FILE}.pdf
	#acroread -toPostScript -size letter -scale 100 -level3 ${FILE}.pdf
	gzip ${FILE}.ps
	@echo "___________________________________________________________"

close:
	@pdfclose --file ${FILE}.pdf

open:
	@pdfopen --file ${FILE}.pdf

neat:
	@rm -f *.bak *.dvi *.log *.out *.aux *.idx *.lof *.lot *.toc *.blg ./Figs/*.fig.bak

prepare:
	@make neat
	@rm -f *.ps *.ps.gz *.pdf

clean:
	@make neat
	@rm -f *.bbl *.ps *.ps.gz *.pdf

